Cell augmentation framework for topological lattices

Maxwell lattices are characterized by an equal number of degrees of freedom and constraints. A subset of them, dubbed topological lattices, are capable of localizing stress and deformation on opposing edges, displaying a polarized mechanical response protected by the reciprocal-space topology of their band structure. In two dimensions, the opportunities for topological polarization have been largely restricted to the kagome and square lattice benchmark configurations, due to the non-triviality of generating arbitrary geometries that abide by Maxwell conditions. In this work, we introduce a generalized family of augmented topological lattices that display full in-plane topological polarization. We explore the robustness of such polarization upon selection of different augmentation criteria, with special emphasis on augmented configurations that display dichotomous behavior with respect to their primitive counterparts. We corroborate our results via intuitive table-top experiments conducted on a lattice prototype assembled from 3D-printed mechanical links.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
